Retroformer: Retrospective Large Language Agents with Policy Gradient Optimization

Recent months have seen the emergence of a powerful new trend in which large language models (LLMs) are augmented to become autonomous language agents capable of performing objective oriented multi-step tasks on their own, rather than merely responding to queries from human users. Most existing language agents, however, are not optimized using environment-specific rewards. Although some agents enable iterative refinement through verbal feedback, they do not reason and plan in ways that are compatible with gradient-based learning from rewards. This paper introduces a principled framework for reinforcing large language agents by learning a retrospective model, which automatically tunes the language agent prompts from environment feedback through policy gradient. Specifically, our proposed agent architecture learns from rewards across multiple environments and tasks, for fine-tuning a pre-trained language model which refines the language agent prompt by summarizing the root cause of prior failed attempts and proposing action plans. Experimental results on various tasks demonstrate that the language agents improve over time and that our approach considerably outperforms baselines that do not properly leverage gradients from the environment. This demonstrates that using policy gradient optimization to improve language agents, for which we believe our work is one of the first, seems promising and can be applied to optimize other models in the agent architecture to enhance agent performances over time.

==> figtext/comparison_curve.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \includegraphics[width=\linewidth]{figs/hotpotqa_curve.pdf}
  \caption{ The agent performances in terms of success rate and average rewards in two environments. We compare our \ourmethod~with ReAct and Reflexion and observe the consistent performance improvement. (The success rate in all environments is shown on the left top.)}
\label{fig: comparison_curve}
\end{wrapfigure}

==> figtext/head.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth, height=5cm]{example-image-a}
    \caption{An overall of our architecture. While frozen LLMs have shown promises as autonomous agents with proper prompts, gaps between language agents learned with \ourmethod~ and frozen agents by prompt engineering towards practical usability are significant.}
    \label{fig:head}
\end{figure}

==> sections/formulation_backup.tex <==


\section{Challenges}
% not designed to handle actions
% Limited Prompt Size, hard to integrate all the historical states. how to describe and summarize?
% heuristic based prompt engineering, systematic methodology is needed
% LLM not editable  or too large to edit/train
% infinite recursion 
Although LLMs are not designed to handle tool use or take actions, it has been observed~\citep{autogpt23,babyagi23,langchain23} that empirically for text-rich environment, especially when the actions and states are accurately described using natural languages, LLMs work surprisingly well. However there are still plenty of challenges applying LLM-based agents. Here we list several below.

\paragraph{Spurious Actions} LLMs are not pre-trained or designed with an action-agent application in mind. Even some restrictions are explicitly specified in the prompt, the LLM model may still generate spurious actions that are not in the action space $\mathcal{A}$.

\paragraph{Limited Prompt Length} LLM itself is stateless. However, in applications it is preferred to empower agents with states or memories for better performance. It has been observed that LLM based agents are easy to run into infinite loops if the states are not handled nicely. Many LLM agents concatenate all the previous state descriptions and actions into the prompt so that LLM as a way to bestow "state" to the LLM. Inevitably this methodology runs into the prompt length issues. As the trajectory grows longer, the prompt runs out of spaces.

\paragraph{Heuristic Prompt Engineering} Even though a lot of paradigms have been proposed to improve LLM agents' performance~\citep{yao2023react,ahn2022can}, there is a lack of systematic methodologies for consistent model refinement. In fact, manual prompt tuning is still widely used in a lot of the application scenarios.

\paragraph{Prohibitive Training} Most of the well-performing LLMs are too large to be fit in just one or two GPUs. It is technically challenging to optimize the LLMs directly as is done in the the classical reinforcement learning setting. In particular, OpenAI has not provided any solution for RL based finetuning. Most of the issues are caused by the fact that LLMs are not pre-trained or designed with an action-agent application in mind.

\section{Intuition}

Compared to the LLM-based action agents, classical RL agents, though not able to handle text-based environments as nicely in the zero shot setting, are able to keep improving based on the feedback and rewards provided by the environment. Popular RL algorithms include Policy Gradient \citep{sutton:nips12}, Proximal Policy Optimization Algorithm (PPO) \citep{schulman2017ppo}, Trust Region Policy Optimization (TRPO) \citep{SchulmanLMJA15}, and Advantage Actor Critic methods \citep{MnihBMGLHSK16}. 

In this draft we are proposing a simple but powerful novel framework to tackle the challenges mentioned above. On one hand, we would like to leverage the classical RL based optimization algorithms such as policy gradient to improve the model performance. On the other hand, our framework avoids finetuning on the LLM directly. The key is, instead of training the LLM directly, we train a reflection LM. The reflection LM takes users' prompt, rewards and feedback from the environment as input. Its output will be prompt for the actual LLM to be consumed. RL algorithms are employed to optimize the weights in the Reflection LM model instead of directly on the LLM. In our framework the weights in the actual LLM is assumed to be fixed (untrainable), which aligns well with the application scenario when the LLM is either too large to tune or prohibited from any tuning. 

Another perspective viewing our framework is, we train a Reflection LM to apply automatic prompt tuning for the LLM agents. In this case, the RL algorithms such as policy gradients are employed to optimize the prompts. Ideally the Reflection LM can help summarize the past "experience", the users' prompt, the environments' feedback into a condensed text with length limit so that it is easier for the LLM to digest. To some extent, in our setting the original LLM can be considered as part of the environment since its parameters are all fixed.


\section{Notation and Formulation}

We denote a large language model (LLM) based agent as a function $\mathcal{L}_{\xi_l}:\mathcal{M}\rightarrow \mathcal{A}$, where $\mathcal{M}$ is the space of prompts, which may include the actual prompts $m^u$ provided by the users, as well as some contextual information $c\in\mathcal{C}$. Here $\mathcal{C}$ is the space of context as a representation of the current state $\mathcal{S}$ returned by the environment $\Omega$. $\mathcal{A}$ is the space of actions. Note the actions taken by most language model based agents are sampled auto-repressively, so $\mathcal{L}$ is a random function. The subscript $\xi_l$ denotes the re-parameterized random variables involved in the sampling process. Another note is, the LLM-based agent itself is stateless. All the states and possible memorization are characterized as text in the prompt. 

The environment is defined as a tuple $(\mathcal{T}_{\xi_o}, \mathcal{R})$. $\mathcal{T}_{\xi_o}: \mathcal{S}\times\mathcal{A}\rightarrow  \mathcal{S}$ is the state transition function, where $\mathcal{S}$ is the space of states and $\mathcal{A}$ is the action space. Here we assume the states and actions are represented using text. Again we used $\xi_o$ to represent the randomness involved in the state transition. For each state $s\in \mathcal{S}$, a reward function is defined as $\mathcal{R}:\mathcal{S}\rightarrow \mathbb{R}$. At each step of the play, the state $s$ is described using natural language, and integrated into the context $c$. In the context, previous states may also be described and embedded to help LLMs making a good guess on the next action to take. As in all the reinforcement learning setting, the final goal is to maximize the cumulative rewards, or returns $G_{cum}=\sum_{t=0}^T R(s_t)$. In many situations, the rewards are sparse, i.e., $R(s_t)$ are mostly zero except very few states. 

The reflection model takes the all the previous states $s_{1,\cdots, t}$, actions $a_{1,\cdots, t}$, rewards $r_{1,\cdots, t}$, and the user prompt $m^u$ as input, and massage those information into a new prompt $m$ to be consumed by the LLM agent:
\begin{align}
\Gamma_{\xi_r, \Theta}: \left[\mathcal{S}_i,\mathcal{A}_i,\mathcal{R}_i,\mathcal{M}^u_i\right]_{i=1}^t\rightarrow \mathcal{M},
\end{align}
where $\xi_r$ stands for the randomness involved in the reflection model, and $\Theta$ is the set of learnable parameters in the reflection model. The goal of the RL optimization is 
\begin{align}\label{eqn:rl-obj}
    &\arg\max_\Theta~~~~ \mathbb{E}_{\xi_l, \xi_o, \xi_r}\left[\sum_{t=1}^T R(s_t)\right]
    ~~~~~~~s.t.~~~~ \nonumber\\
    & 
    s_{t+1} = \mathcal{T}_{\xi_o}\left(s_t, \mathcal{L}_{\xi_l}\circ \Gamma_{\xi_r,\Theta}\left( [s_i, a_i, r_i, m^u_i]_{i=1}^t\right)\right), ~~~~\forall t\in\{1,\cdots, T-1\}
\end{align}

Note that the only learnable parameters are in the retrospective model $M_r$. Since LLM agent model is fixed, it can be considered as a component of the environment. Specifically, if we construct another environment with the transition function $\mathcal{T}'=\mathcal{T}(\mathcal{S}, \bullet)\circ \mathcal{L}: \mathcal{S}\times\mathcal{M}\rightarrow \mathcal{S}$, and the same reward function $\mathcal{R}$, then the objective in \cref{eqn:rl-obj} is just a regular RL optimization so all the popular RL algorithms apply.

% The notations can be further simplified if we denote $\mathcal{F}=\mathcal{T}(\mathcal{S}, \bullet)\circ \mathcal{L}: \mathcal{S}\times\mathcal{M}\rightarrow \mathcal{S}$.

% \hw{not sure if the notation and formulation section is needed. For now I am leaving it there, but we may comment it out if that does not fit the article}
% % Fixed
% % \hw{regarding the naming of the modules. I feel the name "Reflection" is already occupied by other algorithms/papers. Can we think of another name for the paraphrase module? }

% \hw{we also need to make sure our notations are consistent}

==> sections/property.tex <==
\section{Properties}

==> sections/system.tex <==
\section{Implementation}

\subsection{Model}

\subsection{Environment}

\subsection{Communication}

\subsubsection{Prompt Engineering}

\subsection{Parallelization}

==> tables/ablation.tex <==
\begin{table}[ht]
\caption{Agent performances by fine-tuning with environment A offline and then roll out online in environment B (i.e., A+B). ``All'' means training on rollouts from both environments.}
\label{tab:ablation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
                & HotPotQA+HotPotQA & AlfWorld+AlfWorld & All+HotPotQA & All+AlfWorld \\ \midrule
Success rate    &                   &                   &              &              \\
Average reward &                   &                   &              &              \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/results_10.tex <==
\begin{table*}[t]
\centering
 \caption{\textbf{Ablation studies on few-shot recognition}. \ourmethod: our defined model with $N=4$.}
 \label{tab:ablation}
 \centering
 \small \renewcommand{\arraystretch}{1.0}
 \setlength{\tabcolsep}{3pt}
\begin{tabular} {l>{\columncolor{white}[1pt][\tabcolsep]}l>{\columncolor{white}[1pt][\tabcolsep]}ccccc}   %   {l>{\columncolor{white}[3pt][\tabcolsep]}ccccc>{\columncolor{white}[\tabcolsep][3pt]}r}
\toprule
Dataset                  & Settings  & 1 shot  & 2 shots & 4 shots & 8 shots  & 16 shots\\ \midrule
\multirow{6}{*}{\centering Caltech101} 
    &  \ourmethod   & \bm{$89.83\pm 0.33$}  & \bm{$90.67\pm 0.21$}  & \bm{$90.80\pm 0.20$}  & \bm{$91.54\pm 0.33$}  & \bm{$92.24\pm 0.38$}  \\
    &  CoOp   & $87.51\pm 1.02$  & $87.84\pm 1.10$  & $89.52\pm 0.80$  & $90.28\pm 0.42$  & $91.99\pm 0.31$  \\
    &  G     & $88.13\pm 0.36$  & $86.98\pm 1.25$  & $88.45\pm 0.79$  & $90.16\pm 0.22$  & $90.72\pm 0.18$  \\
    &  G+V    & $88.28\pm 0.43$  & $87.72\pm 1.25$  & $88.45\pm 0.30$  & $89.82\pm 0.20$  & $92.00\pm 0.13$  \\
    &  G+E    & $88.91\pm 0.38$  & $90.01\pm 0.22$  & $90.41\pm 0.20$  & $90.60\pm 0.10$  & $91.74\pm 0.42$  \\
    &  M      & $69.78\pm 1.75$  & $71.57\pm 1.59$  & $77.18\pm 2.16$  & $81.77\pm 0.47$  & $86.21\pm 0.20$  \\
    &  M+V    & $66.11\pm 8.29$  & $71.45\pm 3.98$  & $79.30\pm 3.96$  & $86.96\pm 0.78$  & $89.80\pm 0.17$  \\ 
                                    \midrule%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\centering DTD} 
    &  \ourmethod   & \bm{$46.55\pm 2.62$}  & \bm{$51.24\pm 1.95$}  & \bm{$56.03\pm 0.43$}  & \bm{$61.70\pm 0.35$}  & \bm{$65.60\pm 0.82$}  \\
    &  CoOp   & $43.62\pm 1.96$  & $45.35\pm 0.31$  & $53.94\pm 1.37$  & $59.69\pm 0.13$  & $62.51\pm 0.25$  \\
    &  G      & $45.12\pm 1.69$  & $48.39\pm 2.08$  & $54.75\pm 0.48$  & $60.15\pm 0.70$  & $63.59\pm 0.76$  \\
    &  G+V    & $45.90\pm 2.00$  & $48.50\pm 0.99$  & $53.96\pm 0.48$  & $59.69\pm 1.01$  & $63.51\pm 0.66$  \\
    &  G+E    & $46.39\pm 1.00$  & $49.31\pm 0.56$  & $52.99\pm 0.60$  & $60.44\pm 1.64$  & $63.97\pm 0.48$  \\
    &  M      & $13.18\pm 4.57$  & $12.25\pm 3.86$  & $13.00\pm 4.73$  & $20.76\pm 5.42$  & $26.99\pm 1.98$  \\
    &  M+V    & $12.61\pm 5.93$  & $15.11\pm 1.81$  & $20.35\pm 1.33$  & $44.13\pm 2.39$  & $56.85\pm 0.54$  \\ 
\midrule%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \multirow{6}{*}{\centering FOOD101} 
    &  \ourmethod   & \bm{$77.74\pm 0.47$}  &\bm{$77.70\pm 0.02$}  & \bm{$77.21\pm 0.43$}  & \bm{$75.31\pm 0.30$}  & \bm{$77.09\pm 0.18$}  \\
    &  CoOp   & $74.25\pm 1.52$  & $72.61\pm 1.33$  & $73.49\pm 2.03$  & $71.58\pm 0.79$  & $74.48\pm 0.15$  \\
    &  G      & $74.63\pm 0.11$  & $70.15\pm 0.49$  & $70.41\pm 0.46$  & $70.72\pm 0.98$  & $73.68\pm 0.46$  \\
    &  G+V    & $74.83\pm 0.31$  & $70.09\pm 0.85$  & $70.86\pm 0.22$  & $70.80\pm 0.68$  & $73.93\pm 0.35$  \\
    &  G+E    & $75.77\pm 0.62$  & $73.54\pm 0.88$  & $75.82\pm 0.44$  & $72.40\pm 0.50$  & $75.52\pm 0.33$  \\
    &  M      & $52.02\pm 4.86$  & $46.12\pm 1.46$  & $46.86\pm 1.39$  & $53.43\pm 0.88$  & $61.28\pm 0.23$  \\
    &  M+V    & $46.52\pm 1.15$  & $45.95\pm 2.66$  & $53.57\pm 0.83$  & $62.95\pm 0.37$  & $67.63\pm 1.11$  \\ \bottomrule
\end{tabular} 
\end{table*}

==> tables/results_T.tex <==
\begin{table}[ht]
\centering
 \caption{\ourmethod~success rate (succ\%) and average reward in N trials and best-of-$n$ shots reflection sampling scored by the learned reward model in HotPotQA environment. We use F1 score grading as the reward function to evaluate the alignment of the generated output with the expected answer. The standard deviation is calculated for the average F1 scores over 100 tasks.}
 \label{tab:results@T} 
 \centering
 \small \renewcommand{\arraystretch}{1.0}
 \setlength{\tabcolsep}{3pt}
\begin{tabular} {l>{\columncolor{white}[1pt][\tabcolsep]}l>{\columncolor{white}[1pt][\tabcolsep]}ccccc}   %   {l>{\columncolor{white}[3pt][\tabcolsep]}ccccc>{\columncolor{white}[\tabcolsep][3pt]}r}
\toprule
Environment                  & Settings  & 1 shot  & 2 shots & 4 shots \\ \midrule
    \multirow{4}{*}{\centering HotPotQA} 
                                    & N=0 (initial trial) & \multicolumn{3}{c}{---------------------- $34\% / 0.43 \pm 0.46$ ----------------------} \\
                                    & N=1 & $39\% / 0.45 \pm 0.47$  & $42\% / 0.48 \pm 0.46$  & $45\% / 0.52 \pm 0.47$ \\
                                    & N=2 & $42\% / 0.48 \pm 0.46$  & $45\% / 0.52 \pm 0.47
$  & $48\% / 0.54 \pm  0.47$  \\
                                    & N=4 & $50\% / 0.55 \pm 0.48$  & $52\% / 0.58 \pm 0.46$  & $53\% / 0.60 \pm  0.46$ \\
  \bottomrule
\end{tabular}
\end{table}
%45, 48, 52, 53, 55
